Energy-based Proportional Fairness in Cooperative Edge Computing

By executing offloaded tasks from mobile users, edge computing augments mobile user equipments (UEs) with computing/communications resources from edge nodes (ENs), enabling new services (e.g., real-time gaming). However, despite being more resourceful than UEs, allocating ENs' resources to a given favorable set of users (e.g., closer to ENs) may block other UEs from their services. This is often the case for most existing approaches that only aim to maximize the network social welfare or minimize the total energy consumption but do not consider the computing/battery status of each UE. This work develops an energy-based proportional-fair framework to serve all users with multiple tasks while considering both their service requirements and energy/battery levels in a multi-layer edge network. The resulting problem for offloading tasks and allocating resources toward the tasks is a Mixed-Integer Nonlinear Programming, which is NP-hard. To tackle it, we leverage the fact that the relaxed problem is convex and propose a distributed algorithm, namely the dynamic branch-and-bound Benders decomposition (DBBD). DBBD decomposes the original problem into a master problem (MP) for the offloading decisions and multiple subproblems (SPs) for resource allocation. To quickly eliminate inefficient offloading solutions, MP is integrated with powerful Benders cuts exploiting the ENs' resource constraints. We then develop a dynamic branch-and-bound algorithm (DBB) to efficiently solve MP considering the load balance among ENs. SPs can either be solved for their closed-form solutions or be solved in parallel at ENs, thus reducing the complexity. The numerical results show that DBBD returns the optimal solution in maximizing the proportional fairness among UEs. DBBD has higher fairness indexes, i.e., Jain's index and min-max ratio, in comparison with the existing ones that minimize the total consumed energy.

==> DBBD_Journal_bibitems_07Feb2022_v15.tex <==
\begin{thebibliography}{1}
	
\bibitem{vu2022energy}
T.~T. Vu, D.~T. Hoang, K.~T. Phan, D.~N. Nguyen, and E.~Dutkiewicz,
``Energy-based proportional fairness for task offloading and resource
allocation in edge computing,'' in \emph{ICC 2022 - IEEE International
	Conference on Communications}, Conference Proceedings.

\bibitem{Mach2017Mobile}
P.~Mach and Z.~Becvar, ``Mobile edge computing: A survey on architecture and
computation offloading,'' \emph{IEEE Communications Surveys \& Tutorials},
vol.~19, no.~3, pp. 1628--1656, 2017.

\bibitem{mao2017survey}
Y.~Mao, C.~You, J.~Zhang, K.~Huang, and K.~B. Letaief, ``A survey on mobile
edge computing: The communication perspective,'' \emph{IEEE Communications
	Surveys \& Tutorials}, vol.~19, no.~4, pp. 2322--2358, 2017.

\bibitem{Nguyen2014ACM} Diep N. Nguyen and Marwan Krunz, ``A Cooperative MIMO Framework for Wireless Sensor Networks,''
	\emph{ACM Transactions on Sensor Networks (TOSN)}, vol.~10, pp. 1--28, 2014.

\bibitem{el2018edge}
H.~El-Sayed~\emph{et al.}, ``Edge of things: The big picture on the integration
of edge, iot and the cloud in a distributed computing environment,''
\emph{IEEE Access}, vol.~6, pp. 1706--1717, 2018.

\bibitem{du2019enabling}
J.~Du, L.~Zhao, X.~Chu, F.~R. Yu, J.~Feng, and I.~C, ``Enabling low-latency
applications in lte-a based mixed fog/cloud computing systems,'' \emph{IEEE
	Transactions on Vehicular Technology}, vol.~68, no.~2, pp. 1757--1771, 2019.

\bibitem{xing2019joint}
H.~Xing, L.~Liu, J.~Xu, and A.~Nallanathan, ``Joint task assignment and
resource allocation for d2d-enabled mobile-edge computing,'' \emph{IEEE
	Transactions on Communications}, vol.~67, no.~6, pp. 4193--4207, 2019.

\bibitem{liu2019dynamic}
C.~Liu, M.~Bennis, M.~Debbah, and H.~V. Poor, ``Dynamic task offloading and
resource allocation for ultra-reliable low-latency edge computing,''
\emph{IEEE Transactions on Communications}, vol.~67, no.~6, pp. 4132--4150,
2019.

\bibitem{tran2019joint}
T.~X. Tran and D.~Pompili, ``Joint task offloading and resource allocation for
multi-server mobile-edge computing networks,'' \emph{IEEE Transactions on
	Vehicular Technology}, vol.~68, no.~1, pp. 856--868, 2019.

\bibitem{wang2019delay}
J.~Wang, K.~Liu, B.~Li, T.~Liu, R.~Li, and Z.~Han, ``Delay-sensitive
multi-period computation offloading with reliability guarantees in fog
networks,'' \emph{IEEE Transactions on Mobile Computing}, pp. 1--1, 2019.

\bibitem{kumar2010cloud}
K.~Kumar and Y.~H. Lu, ``Cloud computing for mobile users: Can offloading
computation save energy?'' \emph{Computer}, vol.~43, no.~4, pp. 51--56, April
2010.

\bibitem{wang2019cooperative}
Y.~Wang, X.~Tao, X.~Zhang, P.~Zhang, and Y.~T. Hou, ``Cooperative task
offloading in three-tier mobile computing networks: An admm framework,''
\emph{IEEE Transactions on Vehicular Technology}, vol.~68, no.~3, pp.
2763--2776, 2019.

\bibitem{vu2021optimal}
T.~T. Vu, D.~N. Nguyen, D.~T. Hoang, E.~Dutkiewicz, and T.~V. Nguyen, ``Optimal
energy efficiency with delay constraints for multi-layer cooperative fog
computing networks,'' \emph{IEEE Trans. Commun.}, vol.~69, no.~6, pp.
3911--3929, 2021.

\bibitem{wang2021fast}
J.~Wang, J.~Hu, G.~Min, A.~Y. Zomaya, and N.~Georgalas, ``Fast adaptive task
offloading in edge computing based on meta reinforcement learning,''
\emph{IEEE Transactions on Parallel and Distributed Systems}, vol.~32, no.~1,
pp. 242--253, 2021.

\bibitem{wang2021dependent}
J.~Wang, J.~Hu, G.~Min, W.~Zhan, A.~Zomaya, and N.~Georgalas, ``Dependent task
offloading for edge computing based on deep reinforcement learning,''
\emph{IEEE Transactions on Computers}, pp. 1--1, 2021.

\bibitem{liu2020max}
J.~Liu, K.~Xiong, D.~W.~K. Ng, P.~Fan, Z.~Zhong, and K.~B. Letaief, ``Max-min
energy balance in wireless-powered hierarchical fog-cloud computing
networks,'' \emph{IEEE Trans. Wireless Commun.}, vol.~19, no.~11, pp.
7064--7080, 2020.

\bibitem{zhang2019femto}
G.~Zhang, F.~Shen, Z.~Liu, Y.~Yang, K.~Wang, and M.~Zhou, ``Femto: Fair and
energy-minimized task offloading for fog-enabled iot networks,'' \emph{IEEE
	Internet of Things Journal}, vol.~6, no.~3, pp. 4388--4400, 2019.

\bibitem{dong2019energy}
Y.~Dong, S.~Guo, J.~Liu, and Y.~Yang, ``Energy-efficient fair cooperation fog
computing in mobile edge networks for smart city,'' \emph{IEEE Internet of
	Things Journal}, pp. 1--1, 2019.

\bibitem{li2020auction}
F.~Li, H.~Yao, J.~Du, C.~Jiang, Z.~Han, and Y.~Liu, ``Auction design for edge
computation ofloading in sdn-based ultra dense networks,'' \emph{IEEE
	Transactions on Mobile Computing}, pp. 1--1, 2020.

\bibitem{liao2020blockchain}
H.~Liao, Y.~Mu, Z.~Zhou, M.~Sun, Z.~Wang, and C.~Pan, ``Blockchain and
learning-based secure and intelligent task offloading for vehicular fog
computing,'' \emph{IEEE Trans. Intell. Transp. Syst.}, vol.~22, no.~7, pp.
4051--4063, 2021.

\bibitem{zuo2021computation}
Y.~Zuo, S.~Jin, and S.~Zhang, ``Computation offloading in untrusted mec-aided
mobile blockchain iot systems,'' \emph{IEEE Transactions on Wireless
	Communications}, vol.~20, no.~12, pp. 8333--8347, 2021.

\bibitem{nguyen2018price}
D.~T. Nguyen, L.~B. Le, and V.~Bhargava, ``Price-based resource allocation for
edge computing: A market equilibrium approach,'' \emph{IEEE Transactions on
	Cloud Computing}, vol.~9, no.~1, pp. 302--317, 2021.

\bibitem{nguyen2019market}
D.~T. Nguyen, L.~B. Le, and V.~K. Bhargava, ``A market-based framework for
multi-resource allocation in fog computing,'' \emph{IEEE/ACM Transactions on
	Networking}, vol.~27, no.~3, pp. 1151--1164, 2019.

\bibitem{Boyd2004Convex}
S.~Boyd and L.~Vandenberghe, \emph{Convex optimization}.\hskip 1em plus 0.5em
minus 0.4em\relax Cambridge university press, 2004.

\bibitem{narendra1977branch}
P.~M. Narendra and K.~Fukunaga, ``A branch and bound algorithm for feature
subset selection,'' \emph{IEEE Transactions on computers}, no.~9, pp.
917--922, 1977.

\bibitem{jain1984quantitative}
R.~K. Jain, D.-M.~W. Chiu, and W.~R. Hawe, ``A quantitative measure of fairness
and discrimination,'' \emph{Eastern Research Laboratory, Digital Equipment
	Corporation, Hudson, MA}, 1984.

\bibitem{lin2015task}
X.~Lin, Y.~Wang, Q.~Xie, and M.~Pedram, ``Task scheduling with dynamic voltage
and frequency scaling for energy minimization in the mobile cloud computing
environment,'' \emph{IEEE Trans. Services Comput.}, vol.~8, no.~2, pp.
175--186, 2015.

\bibitem{chen2015decentralized}
X.~Chen, ``Decentralized computation offloading game for mobile cloud
computing,'' \emph{IEEE Transactions on Parallel and Distributed Systems},
vol.~26, no.~4, pp. 974--983, 2015.

\bibitem{chen2016efficient}
X.~Chen, L.~Jiao, W.~Li, and X.~Fu, ``Efficient multi-user computation
offloading for mobile-edge cloud computing,'' \emph{IEEE/ACM Transactions on
	Networking}, vol.~24, no.~5, pp. 2795--2808, 2016.

\bibitem{wen2012energy}
Y.~Wen, W.~Zhang, and H.~Luo, ``Energy-optimal mobile application execution:
Taming resource-poor mobile devices with cloud clones,'' in \emph{2012
	Proceedings IEEE INFOCOM}, Conference Proceedings, pp. 2716--2720.

\bibitem{kelly1998rate}
F.~P. Kelly, A.~K. Maulloo, and D.~K.~H. Tan, ``Rate control for communication networks: shadow prices, proportional fairness and stability,'' \emph{Journal of the Operational Research Society}, vol.~49, no.~3, pp. 237--252, 1998.

\bibitem{yu2018green}
Y.~Yu, X.~Bu, K.~Yang, and Z.~Han, ``Green fog computing resource allocation
using joint benders decomposition, dinkelbach algorithm, and modified
distributed inner convex approximation,'' in \emph{2018 IEEE International
	Conference on Communications (ICC)}, Conference Proceedings, pp. 1--6.

\bibitem{miettinen2010energy}
A.~P. Miettinen and J.~K. Nurminen, ``Energy efficiency of mobile clients in
cloud computing,'' \emph{HotCloud}, vol.~10, pp. 4--4, 2010.

\bibitem{liu2015small}
F.~Liu, E.~Bala, E.~Erkip, M.~C. Beluri, and R.~Yang, ``Small-cell traffic
balancing over licensed and unlicensed bands,'' \emph{IEEE Transactions on
	Vehicular Technology}, vol.~64, no.~12, pp. 5850--5865, 2015.

\bibitem{saha2015power}
S.~K. Saha, P.~Deshpande, P.~P. Inamdar, R.~K. Sheshadri, and D.~Koutsonikolas,
``Power-throughput tradeoffs of 802.11n/ac in smartphones,'' in \emph{2015
	IEEE Conf. Computer Communications (INFOCOM)}, Conference Proceedings, pp.
100--108.

\bibitem{mosek2019documentation}
E.~D. Andersen and K.~D. Andersen, ``The mosek documentation and api
reference,'' Report, 2019. [Online]. Available:
\url{https://www.mosek.com/documentation/}

\end{thebibliography}
